Word Embeddings for Chemical Patent Natural Language Processing

We evaluate chemical patent word embeddings against known biomedical embeddings and show that they outperform the latter extrinsically and intrinsically. We also show that using contextualized embeddings can induce predictive models of reasonable performance for this domain over a relatively small gold standard.

==> embedding_correlation.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[scale=0.3]{embedding_sim_correlation.pdf}
    \caption{Correlation analysis on similarity silver set.}
\end{figure}

\begin{table}[tb]
\centering
\caption{Similarity correlation - significance tests (p-values)}
\begin{tabularx}{0.78\textwidth}{@{}lccccccc@{}}
\toprule
{}          & RDKit & CheMU  & PubMed & Drug & Mat2Vec & CheMU & PubMed \\
{}          &       & W2V    & W2V    & W2V  & W2V     & ELMo  & ELMo \\
\midrule
RDKit       &  --- & 0.46 & 0.94 &  0.61 & 0.07 &   0.35 &  0.99 \\
CheMU W2V   &  --- & ---  & 0.00 &  0.00 & 0.00 &   0.00 &  0.00 \\
PubMed W2V  &  --- & ---  & ---  &  0.00 & 0.00 &   0.00 &  0.00 \\
Drug W2V    &  --- & ---  & ---  &  ---  & 0.00 &   0.00 &  0.00 \\
Mat2Vec W2V &  --- & ---  & ---  &  ---  & ---  &   0.00 &  0.00 \\
CheMU ELMo  &  --- & ---  & ---  &  --- &  ---  &   ---  &  0.00 \\
%PubMed ELMo &  0.99 &      0.00 &       0.00 &     0.00 &        0.00 &       0.00 &        0.00 \\
\bottomrule
\end{tabularx}
\end{table}


==> t-test.tex <==
\begin{table}[tb]
\centering
\caption{Student t-tests (similarity). Above: t values, below, p-values. Null hypothesis: the variables are identically distributed.}
\begin{tabular}{@{}lccccccc@{}}
\toprule
{}          & RDKit & CheMU  & PubMed & Drug & Mat2Vec & CheMU & PubMed \\
{}          &       & W2V    & W2V    & W2V  & W2V     & ELMo  & ELMo \\
\midrule
RDKit       &  0.00 &     -4.66 &      -0.43 &    -1.69 &       -6.25 &      -5.57 &       -5.04 \\
CheMU W2V   &  4.66 &      0.00 &       4.64 &     3.98 &       -2.10 &      -1.14 &       -0.52 \\
PubMed W2V  &  0.43 &     -4.64 &       0.00 &    -1.35 &       -6.35 &      -5.63 &       -5.05 \\
Drug W2V    &  1.69 &     -3.98 &       1.35 &     0.00 &       -5.94 &      -5.13 &       -4.46 \\
Mat2Vec W2V &  6.25 &      2.10 &       6.35 &     5.94 &        0.00 &       0.99 &        1.58 \\
CheMU ELMo  &  5.57 &      1.14 &       5.63 &     5.13 &       -0.99 &       0.00 &        0.61 \\
PubMed ELMo &  5.04 &      0.52 &       5.05 &     4.46 &       -1.58 &      -0.61 &        0.00 \\
\bottomrule
\end{tabular}\\
\vspace{0.3cm}
\begin{tabular}{@{}lccccccc@{}}
\toprule
{}          & RDKit & CheMU  & PubMed & Drug & Mat2Vec & CheMU & PubMed \\
{}          &       & W2V    & W2V    & W2V  & W2V     & ELMo  & ELMo \\
\midrule
RDKit       &  1.00 &      0.00 &       0.67 &     0.09 &        0.00 &       0.00 &        0.00 \\
CheMU W2V   &  0.00 &      1.00 &       0.00 &     0.00 &        0.04 &       0.25 &        0.60 \\
PubMed W2V  &  0.67 &      0.00 &       1.00 &     0.18 &        0.00 &       0.00 &        0.00 \\
Drug W2V    &  0.09 &      0.00 &       0.18 &     1.00 &        0.00 &       0.00 &        0.00 \\
Mat2Vec W2V &  0.00 &      0.04 &       0.00 &     0.00 &        1.00 &       0.33 &        0.12 \\
CheMU ELMo  &  0.00 &      0.25 &       0.00 &     0.00 &        0.33 &       1.00 &        0.54 \\
PubMed ELMo &  0.00 &      0.60 &       0.00 &     0.00 &        0.12 &       0.54 &        1.00 \\
\bottomrule
\end{tabular}

\end{table}

